Flows for Flows: Morphing one Dataset into another with Maximum Likelihood Estimation

Many components of data analysis in high energy physics and beyond require morphing one dataset into another. This is commonly solved via reweighting, but there are many advantages of preserving weights and shifting the data points instead. Normalizing flows are machine learning models with impressive precision on a variety of particle physics tasks. Naively, normalizing flows cannot be used for morphing because they require knowledge of the probability density of the starting dataset. In most cases in particle physics, we can generate more examples, but we do not know densities explicitly. We propose a protocol called flows for flows for training normalizing flows to morph one dataset into another even if the underlying probability density of neither dataset is known explicitly. This enables a morphing strategy trained with maximum likelihood estimation, a setup that has been shown to be highly effective in related tasks. We study variations on this protocol to explore how far the data points are moved to statistically match the two datasets. Furthermore, we show how to condition the learned flows on particular features in order to create a morphing function for every value of the conditioning feature. For illustration, we demonstrate flows for flows for toy examples as well as a collider physics example involving dijet events

==> tex/conditional_subsection.tex <==

\subsection{Conditional distributions} 

The distributions that have been studied so far can be extended by introducing rotations and radial scaling. 
A flow for flow model can then learn to move points sampled at one value of the condition such that they follow the distribution defined by another value of the condition. 
The flow for flow model will be conditioned on the difference between the two conditional values in all cases considered here.
All base densities in this section are trained for $32$ epochs and the Flows For Flows model is trained for $12$ epochs.




The power of this approach is illustrated in Fig.~\ref{fig:rotating_circles_density_compare} where a flow for flow model is trained on a distribution composed of four overlapping circles which is conditionally rotated by up to $45$ degrees.
The benefit of a flow for flow model in this setting is that the map between the distributions defined at two different conditional values is continuous and so can be approximated by the invertible neural network that defines the flow for flow.
The map between distributions defined at different values of the condition is also simpler than the map between a standard normal and the conditional distribution.

In contrast the conditional base density has to learn to approximate a discontinuous map from a standard normal distribution to the data directly.
The invertible neural network that defines the base density is a continuous function and so cannot parameterise a discontinuous map.
This means the tails of the four circles distribution are poorly modelled by the base density and results in out of distributions samples as shown in Fig.~\ref{fig:rotating_circles_density_compare}.
\begin{figure}[htbp]
    \centering 
    \includegraphics[width=\textwidth]{figures/f4f_compare.pdf}
    \caption{A flow for flow model trained on a distribution composed from four overlapping circles conditioned on the angle. 
    All models in this figure were trained using maximum likelihood with no regularisation.
    The flow for flow (Flow4Flow) model is given a four circles distribution with no rotation as input.
    }
    \label{fig:rotating_circles_density_compare} 
\end{figure} 

Another way of mapping between two values of the condition is to go via the base density map $f_{\phi'} \circ f_\phi^{-1}$.
In the case of discontinuous distributions this again results in out of distribution samples as shown in Fig.~\ref{fig:rotating_star_colored}.
Further, by color coding the input data it can be seen that the $f_{\phi'} \circ f_\phi^{-1}$ does not have the same continuity as is inherent in the flows for flows model. 
A useful feature of the flows for flows approach is that the learned map has some semantic cohesion without any explicit regularisation.
This is however not guaranteed, which can be addressed by introducing an explicit optimal transport cost, though we find it has negligible impact in these settings.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/f4f_color_compare_star.pdf}
    \caption{
        Color coded input data points are mapped to the same color output point for $15^\circ, 30^\circ$ and $45^\circ$ degree rotations using a Flow For Flow (Flow4Flow) and $f_{\phi'} \circ f_\phi^{-1}$ (Base Distribution).
    } 
    \label{fig:rotating_star_colored}
\end{figure}

The performance of the Flows For Flows approach is replicated in other conditional distributions as shown in App.~\ref*{app:conditional_dists}.

% \sam{The extra plots are just reinforcing the point and are slightly distracting from the main message. Maybe they belong in an appendix? A more compelling figure to show here would be a real life example of some kind, or some kind of conditional distribution where the condition itself is non-trivial. Radial scaling and rotations are quite easy.}
% Similar behaviour can also be seen in conditional densities with radial scaling as shown in Fig.~\ref*{fig:radial_scale_grid}.
% The minimality of the shifts learned by the flows for flows models is also consistent across these distributions as shown in Fig.~\ref*{fig:radial_scale_grid_colored}.
% \begin{figure}
%     \centering 
%     \includegraphics[width=\textwidth]{figures/f4f_radial_grid.pdf}
%     \caption{
%         The conditional distributions produced by a flow for flow model.
%     }
%     \label{fig:radial_scale_grid}
% \end{figure}

% \begin{figure}
%     \centering 
%     \includegraphics[width=\textwidth]{figures/f4f_radial_colored_grid.pdf}
%     \caption{
%         Color encodings of the maps produced by the flow for flow model without any regularisation. 
%     }
%     \label{fig:radial_scale_grid_colored}
% \end{figure}




==> tex/unconditional_subsection.tex <==
\subsection{Unconditional distributions}
To demonstrate the efficacy of the flow for flow method we consider learning maps between arbitrary two dimensional datasets.
In this setting there is no clear benefit in using a flow for flow method, as evidenced by the similarity between using $f_\gamma$ and $f_{\phi'} \circ f_\phi^{-1}$.
This application does, however, demonstrate the ability of the \fff{}  approach to learn maps between different distributions.
In this section all base densities are trained for ten epochs and the Flows For Flows model was trained for 20 epochs.
% In applications where inference time is important then using $f_\gamma$ will have more utility than $f_{\phi'} \circ f_\phi^{-1}$.
% The function $f_\gamma$ can also be parameterised with a convex potential flow, which directly regulates the transport cost of mapping between $x$ and $y$ which results in ... as shown in ...



\paragraph{Learning the identity}
In the simplest case the two data distributions between which we want to map are identical, and as demonstrated in Fig.~\ref*{fig:identity_map} this map can be learned with a flow for flow model.
Using the map $f_{\phi'} \circ f_\phi^{-1}$ is also possible in this setting, but as the base densities are trained separately the resulting map is very far from the identity as shown by the color coding of the input points in Fig.~\ref*{fig:identity_map}.
This could be remedied with joint training of the base densities, but in real world settings the two distributions are likely to be similar~\cite{curtains} and so mapping to an intermediate gaussian representation represents additional and unnecessary computation.
In contrast the flow for flow model learns a close approximation to the identity without any need for regularisation, though this appears to be closely linked to the initialisation of the invertible neural network.

\begin{figure}
    \centering
    % \includegraphics[width=\textwidth]{figures/checkerboard_identity.png}
    % \includegraphics[width=\textwidth]{figures/fourcirc_identity.png}
    \includegraphics[width=0.75\textwidth]{figures/colour_identity.pdf}
    \caption{A flow for flow model trained to learn a map between two $2$D checkerboard (top) and four circle (bottom) distributions. Both models in this figure were trained using maximum likelihood with no regularisation. 
    A Base Transfer refers to using $f_{\phi'} \circ f_\phi^{-1}$.
    Each input point is assigned a color that is then matched to the output point, such that the distance between input and output points can be visualised.
    % \general{Need to work on this figure, make it a pdf, use many more points, and have better titles/ticks.}
    % \johnny{this is also one of the best out of the box, would be nice to have a grid.}
    % \sam{I think for the first version to be put on the arxiv we don't need a grid for this. Rather than going for many toy datasets it would be more interesting to do something real world?}
    }
    \label{fig:identity_map} 
\end{figure}

\paragraph{Different distributions}
A more thorough test of using flows for flows is to learn the transformation between any pair of arbitrary distributions with the same dimensionality. 
% A flow can also learn a map between any two data distributions of the same dimensionality.
In Fig.~\ref{fig:dist2dist_grid} flows for flows are used to transport between three input and four target distributions of varying complexity.
In all cases using the two base distributions directly outperforms the flows for flows, though it should be noted that it is not envisioned that flows for flows would find a practical application to such transformations and the base densities together have double the number of parameters as the Flows For Flows model.
The key point here is that the Flows For Flows approach can be used to find a map between arbitrary distributions, and the performance can be improved with more parameters (see Fig.~\ref{fig:dist2dist_grid_bigger}).
% However, the performance of the flow for flow model can be improved with optimising the flow architecture and hyper-parameters for each configuration. 

% This is demonstrated in Fig.~\ref{fig:checkers_to_circles} where a flow for model is trained to find a map between a checkerboard distribution and a distribution composed from four overlapping circles with a fixed width.
% In this case an L$2$ loss was used to penalise shifts between the input and output of the map $f_\gamma$, and again it can be seen that this map produces a similar distribution to $f_{\phi'} \circ f_\phi^{-1}$ but with a reduced transport cost \general{Need to measure and introduce this}.
% \sam{The top figure is unpenalised and the bottom figure has the L2 cost, but why is the penalised one better?}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/dist2dist_grid}
    % \includegraphics[width=\textwidth]{figures/checkerboard_to_circles_unpenalised.png}
    % \includegraphics[width=\textwidth]{figures/checkerboard_to_circles_penalised.png}
    \caption{Flow for flow models trained to learn a map between various $2$D distributions. The models in this figure were trained using maximum likelihood with no regularisation. 
    % A BDTransfer refers to using $f_{\phi'} \circ f_\phi^{-1}$.
    % Each input point is assigned a color that is then matched to the output point, such that the distance between input and output points can be seen directly.
    % \general{Same as previous plot, need a simple way to reload these dists.
    % Also in principle the base densities here could be the same? This would mean there just needed to be one additional subfigure but would also be a slight pain to make with a special script.
    % }
    }
    \label{fig:dist2dist_grid}
\end{figure}

\subsection{Distance penalty}

As it is possible to regularise or constrain the normalizing flow used to transport data in \fff{} , we introduce an L1-norm distance penalty on the input and output data.
This distance regularisation is trivial to introduce for \fff{}  but non-trivial in the case where two normalizing flows are used to move data from one distribution to another.

To demonstrate its ability to better regularise the overall shift of data we introduce this to \fff{}  trained to learn the identity and compare this to using two normalizing flows and transporting data via encoding to and decoding from the base distribution.
The values are shown in Tab.~\ref{tab:avgdist_identity}.
We can see that out of the box \fff{}  typically learns not to greatly displace the data and learn the identity, however with the introduction of the distance penalty it is almost perfect in learning the identity function. The biggest impact is seen for the concentric circles distribution, as shown in Fig.~\ref{fig:identity_map_pen}.

\begin{table}[h]
    \centering
    \caption{Average translation distance of data transformed with a \fff{}  model, a \fff{}  model with an L1 distance penalty with a weight of 1.0, and by an encoding-decoding with the two normalizing flows used to train the \fff{} .
    The same distribution is used for both the input and output, but two separate normalizing flows are trained for the base distribution. All values are absolute mean translations.
    The datasets marked with $^{\dagger}$ have been run with a different random initialisation.
    Models trained with only the L1 norm distance penalty are shown in the last common to quantify the lower bound of expected performance.
    % \general{Are there other maps we should add this table for?}
    } 
    \begin{tabular}{ r | c c c | c}
        2D dataset & Flow4Flow & Flow4Flow + L1 & Base Density transport & L1 norm only\\
        \hline
        Ring & 0.216 & 0.002 & 0.566 & 0.001\\
        Concentric Rings & 2.184 & 0.003 & 1.108 & 0.001\\
        Four Circles & 0.006 & 0.003 & 1.363 & 0.001\\
        Checkerboard & 0.015 & 0.003 & 1.347 & 0.001\\
        Spirals & 0.185 & 0.003 & 1.410 & 0.002\\
        Star & 0.019 & 0.002 & 0.526 & 0.001\\
        Eight Star & 1.576 & 0.430 & 1.474 & 0.001\\
        \hline
        Ring$^{\dagger}$ & 0.025 & 0.002 & 0.679 & -- \\
        Concentric Rings$^{\dagger}$ & 2.823 & 0.008 & 2.174 & -- \\
        Eight Star$^{\dagger}$ & 0.516 & 0.002 & 1.019 & -- \\
    \end{tabular}
    \label{tab:avgdist_identity}
\end{table}


In general this is not of interest on its own, however it demonstrates the natural tendency of \fff{}  to converge on a simpler transport map. Introducing an additional regularising term in the form of a distance penalty provides improved flexibility and better performance on functions that target the optimal transport map and settings where the input and target distributions are similar. %\general{If we want to look at this for mapping between arbitrary distributions we need to also include a fidelity map that measures how well the transform matches the target. For the first preprint we think what is here is enough.}
\begin{figure}
    \centering
    % \includegraphics[width=\textwidth]{figures/concring_identity_nopen.png}
    % \includegraphics[width=\textwidth]{figures/concring_identity_l1pen.png}
    \includegraphics[width=\textwidth]{figures/colour_identity_pen.pdf}
    \caption{A flow for flow model trained to learn a map between two $2$D concentric ring (top) and two eight star (bottom)  distributions. The Flow For Flow models are trained using maximum likelihood with no regularisation (top) and L1 regularisation (bottom). 
    A Base Transfer refers to using $f_{\phi'} \circ f_\phi^{-1}$.
    Each input point is assigned a color that is then matched to the output point, such that the distance between input and output points can be seen directly.
    % \sam{The base density here is the same in both cases so should just place central figure of lower into the same row as the top.}
    % \sam{In the case of the identity we should compare distance only penalties as well, because in the end this will be the same thing.}
    } 
    \label{fig:identity_map_pen} 
\end{figure}
